Evidential Cyber Threat Hunting

A formal cyber reasoning framework for automating the threat hunting process is described. The new cyber reasoning methodology introduces an operational semantics that operates over three subspaces -- knowledge, hypothesis, and action -- to enable human-machine co-creation of threat hypotheses and protective recommendations. An implementation of this framework shows that the approach is practical and can be used to generalize evidence-based multi-criteria threat investigations.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:disc}


==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:eval}


==> sections/hunting-model.manifold.tex <==

Traditional attack detection and defense mechanisms often operate as separate, loosely-connected activities in threat hunting and mitigation contexts. When a suspicious event is detected in the monitoring data, the conventional course of action is to generate an intrusion alert in order to notify a security analyst about a potential threat. In response to the incident, the analyst correlates the alert to different sources of intelligence (both internal and external to the enterprise) to determine an appropriate mitigation strategy to counter the threat. The outcome is the execution of one or more defensive actions, such as blacklisting a remote DNS domain, patching a software vulnerability, or in more extreme cases, suspending network access to the targeted asset.
%, while a better characterization of the nature and scope of the threat is sought.

\begin{figure}
	\centering
	\begin{subfigure}[h]{0.185\textwidth}
		\includegraphics[width=\textwidth]{figures/orion-traditional}
		\caption{}
		\label{fig:manifold:traditional}
	\end{subfigure}
	~
	\begin{subfigure}[h]{0.275\textwidth}
		\includegraphics[width=\textwidth]{figures/orion-manifold}
		\caption{}
		\label{fig:manifold:HDMF}
	\end{subfigure}
	\caption{Illustration of the high-dimensional decision manifold functor (HDMF) in the context of cyber threat hunting. (a)~Traditional first-order functions in cyber threat hunting. (b)~Linking high-dimensional operations in cyber threat hunting with HDMF.}
\label{fig:manifold}
\end{figure}

This semi-manual process is onerous and requires that cyber combatants connect 
spatially and temporally scattered security alerts in order to comprehend threat scenarios, assess the impact of an attack, and defend against it. Figure~\ref{fig:manifold:traditional} illustrates this concept. In this model, threat detectors are partial functions mapping collected \emph{data} (e.g., network packets, system traces, logs) to security \emph{alerts}, and detection responses are denoted by the hyperplane relating alerts to \emph{defenses}---the protective measures available to the defendant. Such a reactive approach is insufficient for effective threat hunting because (1)~it fails to capture the high-dimensional features of advanced attacks (local, global, and offense contexts), yielding too many false positives, (2)~it imposes a \emph{cognitive overload}~\cite{Kirsh2000} on threat hunters, (3)~it does not resist adversarial manipulation of sensors and threat detection models, and (4)~it misses the larger attack campaign, because defensive actions respond to single, out-of-context events, therefore promoting a ``whack-a-mole'' threat hunting mentality.

To better characterize the dynamics of advanced cyber threats and fuel the threat hunting process, we envision concept-rich, evasion-resistant manifolds as \emph{multi-functors} that define structure-preserving mappings (a.k.a. morphisms) on threat knowledge, hypothesis, and action subspaces. Unlike the \emph{first-order} threat detection and response capabilities of traditional cyber security models, such decision manifolds, depicted in Figure~\ref{fig:manifold:HDMF}, connect cyber-hunting operations in a high-dimensional space---where each subspace comprises many dimensions---thus coping with the cognitive overload problem (by enriching the internal data with threat information that can be used to automatically disprove or accept many types of threat hypotheses) and adversarial targeting (by embedding internal models of the attack scenario into the decision space).

The proposed model introduces three high-dimensional subspaces, which shape  manifold boundaries and augment the threat hunting process with contextual information, evidence-based reasoning, and a defense capability model.

\inlinedsectionitblock{Knowledge Subspace} defines the scope of what is \emph{known} about the \emph{internal} and \emph{external} environments. Internal knowledge includes monitoring events (e.g., firewall and system logs, network packers and flows, system traces), network and assets information (e.g., sensors, services, version, and configuration), and internal threat information (e.g., vulnerability assessment reports, verified threats). External knowledge includes external threat intelligence (e.g., security feeds, threat reports, malicious domains) and security analytics information (e.g., security knowledge graphs, file reputation and analysis services). 

\inlinedsectionitblock{Hypothesis Subspace} defines the domains of \emph{detection hypotheses} and \emph{threat hypotheses}. A detection hypothesis defines an attack proposition (e.g., ``host$_\textnormal{A}$ is vulnerable to reflected server XSS'', ``host$_\textnormal{B}$ and client$_\textnormal{X}$ beacon every two hours''), which can be substantiated by the type of detection analysis employed (cf. Section~\ref{sec::detection-types})---encoding a notion of detection precision or confidence level in the hypothesis. A threat hypothesis embeds the higher-level reasoning performed by threat hunters, serving as cognitive glue and trigger for the next step of the hunting process. Examples of threat hypotheses include propositions about threat type (e.g., ``downloaded binary in client$_\textnormal{Y}$ is trojan$_\textnormal{Z}$'', ``beaconing behavior between host$_\textnormal{B}$ and client$_\textnormal{X}$ is part of a C\amper{}C protocol'')  and impact assessment propositions (e.g., ``clients who accessed host$_\textnormal{B}$'s web server have been infected with trojan$_\textnormal{Z}$'', ``trojan$_\textnormal{Z}$ has spread laterally to other clients in the network'').
%It leverages domain knowledge, or premises, to 

\inlinedsectionitblock{Action Subspace} encodes the space of \emph{defense mechanisms} and \emph{protective measures} available to cyber defendants. Examples of defense mechanisms include proactive monitoring (e.g., update a magnet's policy), blocking (e.g., updating firewall rules), statically analysing deployed software for malware and vulnerabilities (e.g., finding unpatched code clones on OS kernels~\cite{jang:2012sp}), sandboxing (e.g., dynamic analyze suspicious binaries sourced from infected clients~\cite{kirat:2014sec,kirat:2015ccs}), and deploying deceptive responses across the software stack (e.g., network and application-level decoys~\cite{Araujo2014,Araujo2015b}, honeyclient analysis~\cite{Taylor2016}, data redaction~\cite{Araujo2015}). Protective measures include disseminating HDMF specifications across endpoints and sharing hunting outcomes with partners organizations.

\vspace{6pt}\noindent For example, a na\"ive approach to detecting \emph{beaconing} behavior in computer networks is to compute histograms to count the number of communications between peers in a network, raising alerts when the count is above a pre-defined threshold. This is imprecise and leads to the generation of too many false alerts.   
Instead, our approach (cf. Section~\ref{sec::RSC}) generates more accurate detection hypotheses about beaconing behavior by \emph{morphing} discrete network communication events into the frequency domain, leveraging a discrete-time Fourier transform (DTFT) to map the discrete sequence of communication events between pairs of network endpoints to an equivalent-length sequence of equally-spaced events---a complex-valued function of frequency. To eliminate false positives, our analysis enriches this decision model with threat intelligence and domain-specific information that serve to weed out legitimate beaconing behaviors and identify new types of beaconing. Upon verification, the malicious beaconing hypothesis elicits a protective measure harnessed from the action subspace to counter the threat.

\contrib{We plan to systematically investigate these subspace categories, and identify dominant vector spaces for each phase of the attack kill chain, with focus on targeted attacks and advanced persistent threats. The expected outcomes of this effort will enrich TA1 detection analyses, inform TA2 data retention policies, and enable comprehensive evidence-based deliberations for threat hunting and adversarial resistance in TA4.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END
\iffalse
\paragraph{Example 1: False Positive Elimination and Impact Assessment.}
Typically, when the histogram-based detector observes a new beacon, threat hunters attempt to determine whether the offending endpoints are part of a botnet whose remote host acts as the command-and-control (C\&C) server. Once this manual deliberation is completed, a prescriptive defense measure (as simple as a table look up) is deployed (e.g., shutdown the network connection of the compromised client). This process is error-prone, since defensive responses might disrupt the operation of critical services executing legitimate heartbeat protocols, while missing other compromised clients in the network (which evade detection by keeping the amount of communication with the C\&C server below  detection thresholds). 

\paragraph{Example 2: Evading Attacker Elimination.}
If an attacker knows the common reactions to specific attacks, e.g., blocking
one port if attack A is seen. He may try to get his attack classified as attack
A so that only a port is blocked after it is detected.

If the detection system yields that one attack found with 40\% likelihood to be
attack A, 30\% likelihood to be attack B, and 20\% likelihood to be attack C.
More actions can be considered to prevent potential damage if it turns out to
be attack C instead of A.
\fi

==> sections/use-case.tex <==
\section{Application to Threat Hunting Scenarios}

\iffalse
We discuss how ORION performs comprehensive cyber hunting in a sophisticated
attack scenario where an attack group compromises targeted company devices,
gains access to the critical assets, and exfiltrates confidential information by
leveraging various attack techniques, such as XSS attacks, drive-by download
infection, stealthy C\&C communication, and reconnaissance.
\fi

\begin{figure}
  \centering
  \includegraphics[width=1\columnwidth]{figures/attack-scenario.pdf}
  \caption{Attack scenario}
  \label{fig:attack-scenario}
\end{figure}

\inlinedsection{Threat Scenario} Figure~\ref{fig:attack-scenario} depicts an attack campaign that sets up malware distribution servers and C\&C endpoints for attack orchestration and data exfiltration (\tcircled{0}). The targeted attack starts with delivering a crafted web link containing a reflected XSS attack via a spear phishing tactic (\tcircled{1}). When an unsuspecting user is tricked to follow the web link (\tcircled{2}), the vulnerable web server reflects the XSS attack to the user's web browser (\tcircled{3}). The XSS attack redirects the browser to the attacker's malicious web server (\tcircled{4})
which then exploits the browser's vulnerability to install malware
(\tcircled{5}). Once malware infects the user's device, it establishes a communication channel with a C\&C server using DGAs and/or fast-fluxing techniques for further instructions (\tcircled{6}). Malware makes a lateral movement to other devices to locate critical assets in the company networks, e.g., leveraging zero-day exploits (\tcircled{7}). Malware beacons to a C\&C server to report its presence and receive further instructions (\tcircled{8}), and conducts internal reconnaissance to identify and gain access to critical assets (e.g., code repositories) using stolen credentials (\tcircled{9}). Once malware collects confidential information, it exfiltrates the information to a remote server controlled by the attacker (\tcircled{{\footnotesize 10}}).

\iffalse
\subsection{Malicious Domain Name Generation}
DNS is often a bellwether for the health of a network, and monitoring
DNS traffic can uncover a treasure trove of malicious activity.  One
such type of activity is the automatic generation of domain names by
bots. A bot will generate and query a number of random domain names,
only one of which will return a valid IP address in the query
response.  This address is the location of the botnet's command-and-
control server.  These so-called domain name generation algorithms (DGAs) are designed
to make it extremely difficult for defenders to blacklist C\&C
servers.

Figure \ref{fig:uc:dga} shows the threat hunting flow for the
detection of a network client suspected of producing DGA activity.
DNS traffic is collected using a passive tap and analyzed using our
proposed \tthree DGA detector.  The detector is designed to
quickly filter out clients that clearly do not exhibit bot-like
behavior.  This results in the vast majority of network clients being
filtered out.  Furthermore, a detection hypothesis DH$_2$ is generated to validate
if those remaining clients are indeed displaying DGA behaviors.   To validate
the hypothesis, a DGA
validation manifold $\manifold_1$ decides that a more thorough analysis by \tone
DGA analytic $\detector_2$ is necessary (cf.
Section~\ref{sec::detection-types}).  The analytic takes into
consideration more feature-rich historical data to
make an accurate classification with a high confidence level ($cl$).

Once the client is confirmed to be exhibiting DGA behavior, a threat
hypothesis TH$_6$ is generated to determine whether the DGA behavior is
attributed to a known botnet, a known benign behavior, or an unknown
behavior.  The hypothesis is proved or disproved using intelligence
gathered in the security knowledge graph (cf. Section~\ref{sec::skg}).

If the DGA behavior is attributed to a known botnet, or cannot be
attributed to anything, it is added to a case graph, and passed to an
action manifold to determine whether some action should take place
(cf. Section~\ref{sec::pm-responses} for details on responses).  For example, if the
client is found to be a crown jewel, it will be immediately quarantined.



\begin{figure*}[t]
	\centering
	\begin{subfigure}[h]{0.3925\textwidth}
		\includegraphics[width=\textwidth]{figures/orion-dga-hunt}
		\caption{}
		\label{fig:uc:dga}
	\end{subfigure}
	~
	\begin{subfigure}[h]{0.58\textwidth}
		\includegraphics[width=\textwidth]{figures/orion-beaconing-hunt}
		\caption{}
		\label{fig:uc:beac}
	\end{subfigure}
	\caption{Threat hunting cases illustrating (a)~malicious DNS domain name generation hunt, and (b)~beaconing analysis and impact assessment hunts.}
\label{fig:uc:dga-beac}
\end{figure*}

\subsection{From Beaconing to Lateral Movement}
\showOwners{\owner{Fred}}

Cyber attacks often require communication with the outside world in order to
receive commands and exfiltrate data.   As a side effect, attacker-controlled
malware will frequently exhibit beaconing behavior that can be identified
using signal processing algorithms.   This section will extend the formally-defined example introduced in Section~\ref{sec::hunting-model} and complement it with a visual representation of the hunt model.

Figure \ref{fig:uc:beac} shows a possible threat hunting workflow for
beaconing with an emphasis on the generation of threat hypotheses.
The Figure starts with a \tone beaconing
detection DH$_{1}$ (cf. Section~\ref{sec::detection-types}) using our proposed algorithm.  This elicits a knowledge graph exploration (cf. Section~\ref{sec::skg}), which yields three threat hypotheses TH$_{1\textnormal{--}3}$ are generated: (1) the
client is a command-and-control server, (2) the client is a trojan, or
(3) the client is interacting with a malware distribution service.
Each hypothesis is verified using a different mechanism
for demonstration purposes.

The C\&C hypothesis is proved or disproved using the security
knowledge graph ($\verifiers_{2}$ ), similar to the DGA use case. If the beacon is
validated to be a C\amper{C} channel, then an analysis $\hunter_{3}$ is started to
determine if the infected client is part of a larger attack campaign
by generating two more threat hypotheses TH$_{4\textnormal{--}5}$.  The first
hypothesis (TH$_4$) is used to identify whether the infected client is
communicating with other C\amper{C} servers.  This is verified by doing a
dynamic analysis of the malware (if available), or deploying
sandboxes to the infected client to heavily monitor system activity.
TH$_5$ is used to investigate whether there are other hosts infected with
the same malware.  This analysis is done with a historical
analysis to see whether any hosts (1) have contacted the same C\amper{C}
server, (2) downloaded the same software, or (3) are exhibiting
similar behaviors.  Further intelligence gathering can happen by
deploying a dynamic monitoring system to hosts to which the infected
client interacts.

Verification of the trojan hypothesis TH$_2$ is done by a sandbox
analysis of all binaries downloaded by the client in the past few
days.  Once the hypothesis is proven, an overall impact analysis
is conducted, which mirrors the C\amper{C} analysis described above.
Analysis of the malware delivery service hypothesis (TH${_3}$) is done
through an offense context verification that verifies whether any
internal host has downloaded software from the same malware delivery
service.  Once all hosts involved in the attack campaign are identified, ORION
will notify the analyst, and quarantine the assets involved.


\subsection{XSS Detection and Sandbox Analysis}
\showOwners{\owner{Adam/Dhilung}}

The attack scenario described in Figure~\ref{fig:attack-scenario} starts from an
XSS attack triggered by a spear phishing email. The XSS attack is first detected
by the \tthree detector, which produces a low confidence detection hypothesis
that the Client$_\textnormal{1}$ is under an XSS attack. This instantiates a new
case graph and a new workflow. The XSS validation manifold performs \tone XSS
detection analysis to verify the weak detection hypothesis. If the XSS attack is
verified with high confidence, the action manifold forwards the URL used for the
XSS attack to the evasive malware sandbox along with the Client$_\textnormal{1}$
context. The sandbox prepares an execution environment equivalent to the
Client$_\textnormal{1}$ environment and runs dynamic analysis by opening the
URL. The sandbox quickly determines the malicious drive-by-download activity,
the related malware binary, and the attempt of a lateral movement using
harvested honey credentials. In case a zero-day exploit is used for the lateral
movement, the sandbox produces a weak hypothesis of possible lateral movement
only based on the local network activities, which then can trigger a hypothesis
verifier that performs a more detailed sandbox analysis consisting of multiple
networked sandboxes.

After the sandbox analysis, the threat context in the case graph is enriched
with more intelligence and, hence, a more advanced case analysis
manifold is applied, producing more hypothesis verifiers and protective
responses. The protective response, such as quarantining Client$_\textnormal{1}$
can deter the attack earlier.

\subsubsection{Attack Mitigation and Misdirection via Application-Level Deception}

Adversaries typically perform initial reconnaissance missions before
commencing actual attacks. Unfortunately, today's computer systems
(e.g., networks, servers, services, APIs) are too honest and
forthcoming in sharing tremendous amounts of information with
attackers.  Hence, with minimal effort, attackers can glean extremely
valuable information on network topologies, currently running
applications and their version and patch level, as well as potential
vulnerabilities---all without the defender's knowledge.  This
\textit{information asymmetry} favors attackers, allowing them to find
a single weakness, while defenders are faced with the difficult task
of keeping up with all possible vulnerabilities.

We can reverse this imbalance, using our application-level deception
sensors to render vulnerability scanning ineffective.  For example, let's
pretend that the latest threat intelligence report indicates that
there is a new exploit that could allow an attacker to take control of company web
servers (e.g., the Shellshock~\cite{ShellShock} exploit against Apache).  A patch has
been released, but no signature is available for
the company's intrusion detection system.  ORION hypothesizes that
attackers (internally or externally) may be attacking the web server
through this vulnerability and immediately deploys a
honey-patch~\cite{Araujo2015, Araujo2014} to
the running server.

The honey-patch makes the server look vulnerable to the attacker, but
in reality, any exploitation is controlled.  Upon a successful attack
on a web server worker process, ORION drops the infected process into
a transparent sandbox for monitoring.   The initial exploit payload is
extracted and can be used to generate new signatures for the network.
All attacker actions are recorded, and hashes for
the downloaded malware are generated.  ORION uses the hash to see whether the same
malware has been downloaded anywhere else on the network.  Additional
monitoring is deployed to systems found to have downloaded the
malware to determine what other hosts might be involved in the
attacker's lateral movement.    Once all compromised hosts are identified, they are
quarantined simultaneously.
\fi
